A Policy Resonance Approach to Solve the Problem of Responsibility Diffusion in Multiagent Reinforcement Learning

SOTA multiagent reinforcement algorithms distinguish themselves in many ways from their single-agent equivalences. However, most of them still totally inherit the single-agent exploration-exploitation strategy. Naively inheriting this strategy from single-agent algorithms causes potential collaboration failures, in which the agents blindly follow mainstream behaviors and reject taking minority responsibility. We name this problem the Responsibility Diffusion (RD) as it shares similarities with a same-name social psychology effect. In this work, we start by theoretically analyzing the cause of this RD problem, which can be traced back to the exploration-exploitation dilemma of multiagent systems (especially large-scale multiagent systems). We address this RD problem by proposing a Policy Resonance (PR) approach which modifies the collaborative exploration strategy of agents by refactoring the joint agent policy while keeping individual policies approximately invariant. Next, we show that SOTA algorithms can equip this approach to promote the collaborative performance of agents in complex cooperative tasks. Experiments are performed in multiple test benchmark tasks to illustrate the effectiveness of this approach.

==> 01-2Preliminaries.tex <==



\section{Preliminaries}
\subsection{Exploration-exploitation Dilemma.} \label{sec:explorationDilemma}
% To train agents to complete tasks,
An RL algorithm must strike a balance 
between exploration and exploitation in order to train agents effectively\cite{sutton2018reinforcement}.
The exploration-exploitation dilemma has been intensively studied in single-agent problems
for both value-based models and policy-based models.
For value-based models, exploration solutions are $\epsilon$-greedy \cite{szita2008many, sutton2018reinforcement},
Boltzmann exploration \cite{carmel1999exploration, morihiro2006emergence}, probability matching \cite{koulouriotis2008reinforcement} et.al.
The $\epsilon$-greedy is the most common strategy adopted by most MARL algorithms such as QMIX and Fine-tuned Qmix.
On the other hand,
policy-based models \cite{schulman2017proximal, iqbal2019actor, yu2021surprising} heavily rely on stochastic policies and 
entropy regularization to ensure sufficient exploration \cite{williams1992simple, mnih2016asynchronous}.
In multiagent cases, entropy can be calculated on all agents by:
\begin{equation}\label{eq:entropy}
    H  =  \frac{c_H}{N} \sum_{i=1}^{N}  \mathbb{E}_{u_k \sim \pi_i(u_k | o_i)}[-\log \pi_i(u_k | o_i)]
    % = \frac{c_H}{N} \sum_{i=1}^{N}  \sum_{u_k \in \mathcal{U}} -\pi_i(u_k | o_i) \log \pi_i(u_k | o_i)
\end{equation}
where $c_H$ is a coefficient, $\mathcal{A}$ is the set of agents, $N=|\mathcal{A}|$ is the number of agents, 
$\pi_i$ represents agent policies,
$o_i$ represents agent observation and
$\mathcal{U}$ is the set of agent actions, $u_k \in \mathcal{U}$.


In this paper,
we mainly focus on policy-based models.
When analyzing the cause of DR, 
we assume entropy regularization is used because it is adopted in most SOTA policy-based algorithms.
Additionally, we assume $\epsilon$-greedy is used for the analysis of value-based models in Appendix \ref{Policy-Based-Perspective}.


\subsection{Benchmark Environments.}\label{BenchmarkEnvironments}
% 目的
% 基本结构（加图）
% 超越人的认知
% 

% decomposite complicated multiagent tasks
% and then reconstruct them by sequentially arranged levels.
% Alternatively speaking, agents are encouraged only if their action benefits the whole team.

% FME 
% FME is to
% find a convenient way to identify the \textbf{weakness} of a given MARL algorithm.
% to conveniently identify the \textbf{weakness} of a given MARL algorithm.
% But in this paper, the primary purpose of FME is to
% help analyze the DR problem both theoretically and experimentally.

\subsubsection{Fast Multiagent Evaluation (FME).}
To help analyze the Diffusion of Responsibility problem,
we designed a diagnostic environment named Fast Multiagent Evaluation (FME).
 

FME is designed as a test environment that 
uses \textbf{independent and sequentially arranged levels}
to identify the weakness of given MARL algorithms.
Each level is an abstract mini-task, e.g., multiagent multi-armed bandit problem \cite{sutton2018reinforcement}.
Such design enables us to theoretically analyze issues that surface in experiments.

FME levels only provide \textbf{team reward} to increase difficulty and
to fully expose underlying issues of MARL algorithms.
Moreover, by only using team reward FME encourages agents to behave cooperatively rather than selfishly.
% In other words, FME only encourages agents to satisfy team goals.

The following levels are needed to analyze the DR issue,
each of them requires only \textbf{single-step} decision:

\textbf{Lv-A}: Finding a static action with reward.
Agents need to find a predefined action $u^\alpha\in \mathcal{U}$ that leads to reward.
Reward $R_A=N_{\mathcal{A}}(u^\alpha)/N$,
where $N_{\mathcal{A}}(u^\alpha)$ counts the number of agents selecting $u^\alpha$. 
The optimal joint policy is for all agents to simply choose $u^\alpha$, 
and the optimal reward expectation is $\mathbb{E}\left(R_A|\boldsymbol{\pi}^*\right)=1$, 
where $\boldsymbol{\pi}^*$ is the optimal joint action.

\textbf{Lv-B}: Multiagent variant of the \textbf{multi-armed bandit} problem.
After every agent has selected an arm on the bandit,
a random arm $u^\beta \in \mathcal{U}$ is sampled from a predefined constant distribution $p_\beta(u)$.
Reward is $R_B=N_{\mathcal{A}}(u^\beta)c_\beta/N$,
where $c_\beta$ is a constant and $N_{\mathcal{A}}(u^\beta)$ counts the number of agents choosing the $u^\beta$ arm.
The optimal solution (proof in Appendix \ref{lvb-reward}) is all agents selecting
the arm with highest probability according to $p_\beta(u)$.
To scale optimal reward expectation $\mathbb{E}\left(R_B|p_\beta(u), \boldsymbol{\pi}^*\right)$ at 1,
the constant $c_\beta=1/{\underset{u}{\mathrm{max}}[p_\beta(u)]}$.

\textbf{Lv-C}: Responsibility assignment challenge.
Agents are rewarded for selecting a predefined constant action $u^\gamma$ which has a maximum capacity $N-1$.
If all $N$ agents choose $u^\gamma$,
then the capacity of $u^\gamma$ exceeds and reward turns zero.
Informally, $u^\gamma$ can be seen as a fragile bridge that collapses under exceeding weight.
Most agents are responsible for crossing the bridge to reach the destination,
but a minority of agents are responsible for choosing otherwise for the overall interests of the team.

Formally, the Lv-C reward is:
\begin{equation}\label{lvc-reward}
    R_C= \begin{cases}{N_{\mathcal{A}}\left(u_{\gamma}\right)}/{(N-1)}, 
        & 0\le N_{\mathcal{A}}\left(u_{\gamma}\right)<N \\ 0, 
        & N_{\mathcal{A}}\left(u_{\gamma}\right)=N\end{cases}
\end{equation}
where $N_{\mathcal{A}}(u^\gamma)$ is the number of agents selecting constant action $u^\gamma$. 
The optimal reward expectation is $\mathbb{E}\left[R_C|\boldsymbol{\pi}^*\right]={N_{\mathcal{A}}(u^\gamma)}/{(N-1)}=1$
when $N_{\mathcal{A}}\left(u_{\gamma}\right)=N-1$.

Other properties of FME include:
\begin{itemize}
    \item All levels share the action space $\mathcal{U}$, but each level interprets $\mathcal{U}$ differently.
    \item Agents only observe the level indices and one-hot agent identities, which is already sufficient for optimizing policies.
    \item By configuring predefined parameters such as $u^\alpha$, $p_\beta(\cdot)$, $u^\gamma$ differently, 
    each type of level can be used multiple time in a task setting. 
    \item We use a tag such as \textit{1A2B4C} to describe a FME task. 
    E.g, tag \textit{1A2B4C} represents a FME task composed by one Lv-A, two Lv-B and four Lv-C levels with different configurations.
    Detailed parameters are displayed in Appendix \ref{appendix:FMEtable}.
    
\end{itemize}


\begin{table}[!t]
    \vspace{-0.5cm}

    \centering
    \setlength{\tabcolsep}{0.5mm}{
        \begin{tabular}{ccccccccc}
        \toprule
        \tiny{          }   & \tiny{$N$=3}    & \tiny{$N$=5}     & \tiny{$N$=6}    & \tiny{$N$=7}    & \tiny{$N$=8}      & \tiny{$N$=15}    & \tiny{$N$=25}      & \tiny{$N$=40}         \\
        \midrule
        \tiny{PPO-MA         } & \tiny{1.00} & \tiny{1.00}  & \tiny{0.87} & \tiny{0.00} & \tiny{0.00}  & \tiny{0.00}   & \tiny{0.00}   & \tiny{0.00}      \\
        \tiny{Fine-tuned Qmix} & \tiny{1.00} & \tiny{1.00}  & \tiny{1.00} & \tiny{1.00} & \tiny{0.95}  & \tiny{0.85}   & \tiny{0.27}   & \tiny{0.16}   \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{
        The average rewards $R_C$ in Lv-C evaluation.
        Trained and tested in FME diagnostic environment with setting \textit{1A4B2C}.
        (only Lv-C reward is displayed, optimal reward of Lv-C is 1). 
    }
    \label{lvc-problem-intro}
    \vspace{-0.4cm}
\end{table}




\subsubsection{ADCA.}
The Asymmetric Decentralized Collective Assault (ADCA)
benchmark is a swarm combat environment modified and 
improved from \cite{fu2022concentration}.
As shown in Fig.\ref{fig:TwoStagePR-ADCA}, in ADCA, two asymmetric teams compete with each other.
The RL-controlled team has $N=50$ agents,
the enemy team that is controlled by script AI.
The enemy team has more agents ($N' \in [120\%N, 150\%N]$) and weapon advantage,
see Appendix \ref{appendix:adca} for ADCA details.

\subsection{Base Algorithms.}
Following algorithms are used in analysis and experiments:
\begin{itemize}
    \item Fine-tuned Qmix by \citeauthor{hu2021rethinking}. Value-based algorithm.
    \item PPO-MA, similar to the model proposed by \citeauthor{yu2021surprising}, but with action masking and input shaping tricks removed. Policy-based algorithm.
    \item Conc4Hist by \citeauthor{fu2022concentration}. Policy-based algorithm.
\end{itemize}


==> 01Intro.tex <==
\section{Introduction}

% 逻辑线：
% MARL
% 对MARL某些特性的认识尚不完善
% 我们发现一个新问题DR, 特性高度概括
% 联系social psychology
% 独特之处

% 还缺少的点
% 测试的问题
% 普遍性的问题（env选择）, 现有对应的解决方法是task-specific
% PR只用于训练阶段 CTDE
% 作为一个增强手段，需要宿主algorithm，对比方法的问题
% 超越人的认知


% MARL
Recent years have witnessed a growing academic interest in MultiAgent Reinforcement Learning (MARL),
and researchers have proposed a significant number of MARL algorithms to explore the potential of cooperative AIs in many cooperation tasks,
e.g. Starcraft Multi-Agent Challenge (SMAC) \cite{vinyals2017starcraft, usunier2016episodic, lowe2017multi, chen2019crowd, deka2021natural, agarwal2019learning},
Hide-and-Seek with tools \cite{baker2019emergent},
MAgent \cite{rubenstein2014programmable, zheng2018magent, diallo2020multi},
joint-navigation, predator-prey \cite{lowe2017multi} and football \cite{Chenghao2021Celebrating}.
Both policy-based methods \cite{lowe2017multi, iqbal2019actor, yu2021surprising} and 
value-based methods \cite{sunehag2017value, rashid2018qmix, son2019qtran} 
play an essential role in the progress of MARL algorithms.

% 对MARL某些特性的认识尚不完善，泛化性匮乏，不能更好地支持多种任务
Nevertheless, the study of MARL is still far from reaching its ambition.
Firstly, % training a large-scale multiagent team is difficult.
relatively little research investigates general MARL solutions for large teams with more than 30 agents.
On the one hand, 
simplified grid-based simulation limits the generalization ability of models developed in discrete environments such as MAgents,
On the other hand, 
sophisticated benchmarks such as SMAC (maps allowing up to $27$ agents) are not considering large-scale multiagent teams.
Secondly,
multiagent problems, compared with the single-agent equivalence,
still have underlying issues that have not yet been identified, 
because multiagent interaction grows extremely complicated as the number of agents grows.
% For example,
% there is a lack of principle of choice between value-based and policy-based method except for empirical evidence.
% before \cite{yu2021surprising} SMAC was believed to be a .
% Before \cite{de2020independent, yu2021surprising},
% most investigation of value-based and policy-based approaches only focus on very specific types of problems,
% and  was believed to be less effective than off-policy models in SMAC.


% discrete 2D environments cannot reflect 复杂任务中的智能体精细互动
% studies developed under discrete 2D simulations are not 
% while MAgent discrete large-scale simulations
% have problem in generalizing and exposing problems in continuous space,


% 我们发现一个新问题DR, 特性高度概括
This paper reports a newly discovered problem
that surfaces in the multiagent learning process of sophisticated cooperative tasks.
In both value-based and policy-based MARL algorithms,
agents have to explore before they can find better policy or more precise state value estimation,
and to address the exploration-exploitation dilemma \cite{yogeswaran2012reinforcement}.
More specifically, value-based algorithms use $\epsilon$-greedy \cite{szita2008many},
and policy-based algorithms have stochastic policies
implemented entropy regularization that drives agents to explore \cite{schulman2017proximal}.
However, 
note that those measures completely inherit from single-agent RL models
without considering any potential problems which are unique to multiagent systems.
In this paper, we reveal that measures against the exploration-exploitation dilemma during MARL training 
can cause failure in responsibility negotiation between agents.
When a large number of agents are learning to cooperate,
the responsibility of carrying out essential minority behaviors is often neglected by ALL agents.
Furthermore, as the number of agents increases, 
this problem will deteriorate and become even more significant.

% 名字源自social psychology
We borrow a term from the social psychology domain,
Diffusion of Responsibility (DR) \cite{darley1968bystander},
to name this effect because they share similarities in many ways.
In social psychology, 
the Diffusion of Responsibility effect is also known as the bystander effect.
It attempts to explain a crowd's reaction in situations
where help is needed by one (or a few) bystander(s),
e.g., pedestrian fainting, a person in danger of drowning, etc.
The DR problem shows that, in general,
the willingness of individuals to provide help decreases with the number of bystanders.
Psychologists illustrate that all bystander agents struggle
between taking responsibility and staying out of trouble.
When only one agent is present, 
it takes full pressure of the responsibility to intervene.
However, when multiple agents are present, 
no agents prefer to intervene because the responsibility is diffused among agents, 
then overwhelmed by the motivation of staying away from troubles.

% 独特之处
But despite the superficial similarities, 
the underlying mechanism of the DR problem in MARL is different from that in the psychology domain.
We emphasize that
the mechanism of the DR problem is rooted in the exploration-exploitation dilemma \textbf{instead of} agents' egoist or selfishness.
The MARL DR problem exists even if agents are rewarded as a team (instead of individuals),
or reward decomposition methods such as Qmix \cite{rashid2018qmix, hu2021rethinking} are adopted.
Alternatively speaking,
we stress that the MARL DR problem is irrelevant to the way the reward is given (team reward or individual rewards), 
nor the way the credit is assigned (with or without value decomposition techniques).


The main contributions of this paper are:
\begin{itemize}
\item We theoretically analyze the feature and the cause of the DR effect 
    in FME (a multiagent environment to test basic cooperative behaviors).
\item We carry out experiments with various algorithms, 
    including fine-tuned Qmix \cite{hu2021rethinking}, Conc4Hist \cite{fu2022concentration}, and PPO-MA,
    to shed light on the properties of the DR effect, which are consistent with the theoretical analysis.
    We also provide an empirical signature to identify the existence of the DR impact.
\item We propose a Policy Resonance approach to resolve the DR problem 
    under the Centralized Training with Decentralized Execution (CTDE) paradigm.
    Policy Resonance is \textbf{not} an independent algorithm,
    instead, it can be flexibly implemented on most existing SOTA host algorithms,
    e.g., multiagent PPO, Fine-tuned Qmix, and Conc4Hist et.al.
\item We implement our PR method on algorithms, including PPO-MA and 
    Conc4Hist to demonstrate the effectiveness of our PR method 
    on multiple benchmarks, including FME (a small diagnostic multiagent benchmark) and ADCA (a complex swarm combat environment) \cite{fu2022concentration}.

\end{itemize}






==> 02CauseOfDR.tex <==
\section{Brief Analysis of the DR Problem}\label{sec:Analysis}


% Lv-c 是同类问题的一个缩影，如何体现这点呢？
Without appropriate management,
a team with abundant agents can fail to complete simple tasks 
that could have been done by just a few agents.
In this paper, 
we illustrate the DR problem using \textit{FME's responsibility assignment challenge (Lv-C level) in Section \ref{BenchmarkEnvironments}}.
The ideal joint policy is for most team agents to choose the $u^\gamma$ action,
while a minority of agents choose actions other than $u^\gamma$.
And the optimal policy is for all but one agent to constantly choose $u^\gamma$.
A misleading trap policy is that all agents become addicted to action $u^\gamma$ 
and eventually exceeding the limited capacity.

% a problematic result is all agent 
% Evaluating PPO-MA, Fine-tuned Qmix, and PR-enhanced PPO-MA 
% in the FME diagnostic environment.
% FME setting: \textit{1A4B2C}. Algorithm: PPO-MA.



\begin{figure}[!t]
    \vspace{-0.6cm}
    \centering
    \includegraphics[width=\linewidth]{img/PersonalityDevelop.pdf}
    \caption{
        Six individual experiments from Table.\ref{lvc-problem-intro},
        showing the preference development toward $u^\gamma$ of the individual agent in 
        in an FME Lv-C (last Lv-C in \textit{1A4B2C} sequence).
        Using $\pi_i(u_{\gamma})-\frac{1}{N}\sum_{j \in \mathcal{A}}\pi_j(u_{\gamma})$
        to describe the preference of each agent compared with the team average.
    }
    \vspace{-0.4cm}
    \label{fig:PersonalityDevelop}
    \end{figure}

We train agents in FME diagnostic environment with sequential setting \textit{1A4B2C} with
PPO-MA (representing policy-based algorithm) and Fine-tuned Qmix (representing value-based algorithm), respectively.
Results in Table.\ref{lvc-problem-intro} show that 
PPO-MA is misled into the capacity-exceeding trap when the $N \ge 6$.
Fine-tuned Qmix survives more agents but still fails when $N \ge 15$.

Focusing on \textbf{policy-based} PPO-MA algorithm,
we sample 6 individual experiments with $N=3,5,6,7$ 
and illustrate the policy development process of agents in Fig.\ref{fig:PersonalityDevelop}.
To investigate how agents negotiate responsibility about $u^\gamma$,
we use $f(\pi_i) = \pi_i(u_{\gamma})-\frac{1}{N}\sum_{j \in \mathcal{A}}\pi_j(u_{\gamma})$
to describe agents' preference towards $u^\gamma$.
Fig.\ref{fig:PersonalityDevelop} shows that, when $N \le 5$,
agents successfully negotiate on a optimal responsibility assignment plan 
by making \textit{one of the team agents to give up its $u^\gamma$ preference}.
However, when $N=6$ the negotiation fails randomly when the experiment is repeated.
And $N \ge 7$ makes the cooperation impossible.

Next we briefly analyze the reason that policy-based PPO-MA falls into trap in this task:
At the beginning of the training process,
the agents are initialized with random and high-entropy policies,
preferring each action (including $u^\gamma$) almost equally \cite{saxe2013exact, mcelreath2020statistical}.
Let $\varPi_0 = \underset{i}{\operatorname{max}} \pi_i (u_{\gamma}|o_{i} )$ 
be the max probability (among agents) of selecting $u^\gamma$.
Since the initial policy is random, then $\varPi_0 \approx \frac{1}{n_k}$,
where $n_k = |\mathcal{U}|$ is the size of action space.

\textbf{(1).} In the beginning,
the capacity-exceeding penalty has a very low triggering probability $P_{plt}$:
\begin{equation}\label{init}
P_{plt} = P\left[N_{\mathcal{A}}\left(u_{\gamma}\right)=N |\boldsymbol{\pi} \right] 
        = \prod_{i=1}^{N} \pi_i (u_{\gamma}|o_{i} ) 
        \le \varPi_0^N
\end{equation}
e.g., when $n_k=10$, $N=15$ and then $P_{plt}\approx 10^{-15}$, 
meaning that only one capacity-exceeding sample is expected within $10^{15}$ samples.
Unless the number of agents $N$ is small enough,
the learning algorithm cannot notice the capacity-exceeding trap at the beginning.
From another perspective,
the learning algorithm also \textbf{cannot distinguish an Lv-C from an Lv-A at the initial stage}
due to the lack of samples with the capacity-exceeding penalty.
Therefore, the algorithm will encourage all agents to select $u_{\gamma}$,
increasing $\pi_i (u_{\gamma})$ gradually and synchronously $\forall i\in \mathcal{A}$.

\textbf{(2).} 
Then we prove that when $N$ is large enough,
agents cannot stop and reverse the increase of $\pi_i (u_{\gamma})$ unless influenced by entropy regularization.
Firstly, find the necessary conditions for $\pi_i (u_{\gamma})$ to stop growing.
For clarity, we shorten 
$N_{\mathcal{A}}\left(u_{\gamma}\right)=N_{\gamma}$ and shorten $\pi_i (u_{\gamma}|o_i)=\pi_{i\gamma}$.
For an agent $i$, the growth of $\pi_{i\gamma}$ will be stopped and reversed 
when larger $\pi_{i\gamma}$ benefits the team reward no more:
\begin{equation}\label{eq:partial}
    \begin{split}
        \frac{\partial \mathbb{E}[R_C(\boldsymbol{\pi})] }{\partial \pi_{i\gamma}} < 0
    \end{split}
\end{equation}
And from Eq.\ref{lvc-reward}:
\begin{equation}\label{eq:new_exp}
\begin{split}
    \mathbb{E}[R_C(\boldsymbol{\pi})] 
    &= \sum_{k=0}^{N-1} \frac{k}{N-1} P[N_{\gamma}=k] + 0 \cdot P[N_{\gamma}=N] \\
    &= \sum_{k=0}^{N} \frac{k}{N-1} P[N_{\gamma}=k] - \frac{N}{N-1} P[N_{\gamma}=N] \\
    &= \frac{1}{N-1} \sum_{j=1}^{N} \pi_{j\gamma} - \frac{N}{N-1} \prod_{j=1}^{N} \pi_{j\gamma}
\end{split}
\end{equation}
From Eq.\ref{eq:new_exp} and Eq.\ref{eq:partial}:
\begin{equation}\label{eq:xx0}
    \begin{split}
        \frac{\partial \mathbb{E}[R_C(\boldsymbol{\pi})] }{\partial \pi_{i\gamma}} = 
        \frac{1}{N-1} - \frac{N}{N-1} \prod_{j\in[1,N], j\neq i} \pi_{j\gamma} < 0
    \end{split}
\end{equation}
\begin{equation}\label{eq:xx1}
    \begin{split}
        \sum_{j\in[1,N], j\neq i} \log \pi_{j\gamma} > -\log N
    \end{split}
\end{equation}
Define a probability $\varPi_{i\gamma}$ to simplify Eq.\ref{eq:xx1}, s.t.:
\begin{equation}\label{eq:xx2-1}
    \log\varPi_{i\gamma}=\frac{1}{N-1}\sum_{j\in[1,N], j\neq i} \log \pi_{j\gamma}
\end{equation}
% $\log\varPi_\gamma$ as the team agent average at LHS:
From Eq.\ref{eq:xx1} and Eq.\ref{eq:xx2-1} we have:
\begin{equation}\label{eq:xx2-2}
\begin{split}
    \varPi_{i\gamma} > N^{-\frac{1}{N-1}}
\end{split}
\end{equation}
Because of Eq.\ref{eq:xx2-1} and the monotonicity of the log function,
there exists at least one agent $m\in [1,N], m \neq i$ that satisfies $\pi_{m\gamma} \ge \varPi_{i\gamma}$,
therefore:
\begin{equation}\label{eq:xx3}
\begin{split}
    \pi_{m\gamma}  > N^{-\frac{1}{N-1}}
\end{split}
\end{equation}
Unfortunately, as $N$ increase, Eq.\ref{eq:xx3} becomes impossible to be satisfied:
\begin{itemize}
    \item RHS increases and approaches 1, $\lim_{N \to \infty} N^{-\frac{1}{N-1}} = 1$. E.g., when $N=15$, RHS = 0.824; $N=50$, RHS = 0.923.
    \item LHS is limited by entropy regularization in Eq.\ref{eq:entropy}, Section \ref{sec:explorationDilemma} assumption.
    In this case, entropy loss prevents $\pi_{j\gamma}$ from 
    getting closer to 1 (policy becoming deterministic) for all agents.
    % policy $\pi_{j}(\cdot)$ from becoming deterministic.
\end{itemize}
Therefore, we can always find $N_{max}$ such that if $N>N_{max}$,
then Eq.\ref{eq:xx3} cannot be satisfied (by any agent),
consequently, Eq.\ref{eq:partial} cannot be satisfied.
Therefore,
agents $i$ will always race each other to increase
the probability $\pi_{i\gamma}$ under the regularization of entropy,
which well explains the preference development 
in failed experiments in Fig.\ref{fig:PersonalityDevelop}.

% 与单智能体的常识相悖
This result is counterintuitive, 
it is irreconcilable with our single-agent RL knowledge because this is a phenomenon \textbf{unique to multiagent RL} algorithms.
Recall that we are using team rewards to train agents,
the environment only encourages agents to act cooperatively instead of selfishly.
However,
while any agent can greatly benefit from switching their responsibility 
from majority action $u^{\gamma}$ to minority actions $u^{-\gamma}$,
none of them will actually do that due to this Diffusion of Responsibility (DR) problem.

Now we have reached the core of the DR problem.
We cannot simply blame the DR problem solely on entropy regularization and
believe the DR problem exists only in policy-based algorithms.
In fact,
\begin{itemize}
    \item The DR problem also exists when \textbf{value-based} algorithms are applied. (Table.\ref{lvc-problem-intro} and Fig.\ref{fig:DRWithMoreAgents} Fine-tuned Qmix).
    \item The DR problem originates from \textbf{$\epsilon$-greedy} in the case of value-based algorithms. (See Appendix \ref{Policy-Based-Perspective}).
    \item Entropy regularization and $\epsilon$-greedy are both measures to solve the exploration-exploitation dilemma.
\end{itemize}
With these clues,
we can propose a much more intuitive and general explanation:

The exploration behavior of agents has a significant influence on each other in MARL,
but concurrent MARL learners cannot correctly perceive this influence.
From the perspective of a MARL learner, 
this mutual influence caused by \textbf{internal} exploration is mistakenly perceived as
\textbf{external} environment characteristics.
This bias of perception eventually leads to failure in responsibility negotiation.
E.g.,
MARL learners \textbf{cannot correctly distinguish an Lv-C from an Lv-B (multi-arm bandit)} in FME,
because the learners mistakenly regard the Lv-C $u^{\gamma}$ action as a bandit arm that fails randomly,
not knowing that the randomness is actually caused by the \textbf{internal} exploration.
In conclusion,
the multiagent exploration strategy is the root of the DR problem,
and it is more reasonable to trace the cause of the DR problem down to the exploration-exploitation dilemma.



% Current MARL models an agent has full autonomy
% during training, one agent's exploration influence other agents perception
% towards the environment,
% sometime blaming the randomlicity caused by exploration on the environment itself.
% E.g., from the view of the learner,
% it cannot tell the difference from Lv-C from Lv-B (multi-arm bandit),
% because the randomlicity caused by exploration is perced as a virtual arm on a brandit that fails occationaly.
% can disrupt the exploration






\section{The Non-triviality of the DR Problem}
In previous sections,
we theoretically analyze the DR problem in FME diagnostic environment,
but an important question is left unanswered:
\begin{enumerate}
    \item \textit{Is DR a general problem 
    that can disguise and merge itself into sophisticated MARL tasks 
    such as Starcraft, ADCA, et al.,
    or is it simply a phenomenon that exists only in our diagnostic environment?}
    \item \textit{Can existing algorithms solve the DR problem?}
    \item \textit{For a black box MARL task, do we need to identify DR problems before dealing with them?}
\end{enumerate}


First, the DR problem is a general issue in MARL.
The FME diagnostic environment is an abstraction and reflection of actual scenarios 
agents encounter in complicated cooperation tasks such as SMAC, ADCA, etc.
The DR problem in FME seems easy to solve via reward hand-crafting,
but such a solution cannot handle the DR issue 
hidden behind the scenarios FME reflected.
For example,
observation range is limited in both SMAC and ADCA,
a minority of agents need to patrol unknown area
while the majority of them deal with already known enemies.
Moreover,
in SMAC RL algorithms make decisions periodically instead of constantly.
If an enemy $X$ is killed halfway through a decision step,
agents with the \textit{Attack-$X$} order become idle 
(even if there is another enemy $Y$ firing at them).
In this case,
the best policy is for the majority of agents to instantly turn to $Y$
when the HP of $X$ is low, 
leaving only a minority of agents to finish off $X$.
Similar scenarios also exist in ADCA.
When a group of agents is being pursued by enemies with numerical superiority,
the majority of agents need to retreat and regroup somewhere with terrain advantage,
while a minority of agents have to stay behind to slow down pursuers 
(by eliminating several frontline enemies).
When the number of agents $N$ is large,
all those scenarios can trigger the DR problem we have seen in FME Lv-C.

Second, 
there are no concurrent and non-task-specific methods against the DR problem.
It is difficult, if not impossible, 
to apply methods such as reward-crafting to these sophisticated scenarios above.
Furthermore,
there may be forms of cooperation actions
beyond the human cognition ability in large multiagent systems, 
e.g., the cooperative behaviors of insects in a swarm.
If a multiagent system grows large enough,
MARL algorithms will inevitably produce cooperative behaviors beyond our understanding.
If DR problems occur in such systems,
we can only solve them with \textbf{general and non-task-specific} methods.


Third,
as this section has revealed, 
it is difficult to analyze DR problems rigorously in multiagent systems.
However,
\textbf{if a general approach can be found to solve the DR problem 
without damaging the original algorithm structure and performance,
we can safely apply this approach without even knowing the existence of the DR problem.}
The next section proposes a Policy Resonance approach to achieve this objective.
















==> 03PersonalityRF.tex <==







\section{Policy Resonance}

\begin{figure}[!t]
    \vspace{-1cm}
        \centering
        \includegraphics[width=0.8\linewidth]{img/resonance_2.pdf}
    \vspace{-0.1cm}
    \caption{The policy resonance procedure.}
        \label{fig:PolicyResonance}
    \vspace{-0.5cm}
    \end{figure}
    
\begin{figure*}[!t]
    \vspace{-0.7cm}
    \centering
    \includegraphics[width=0.8\linewidth]{img/PPOMA+PR.pdf}
    \vspace{-0.1cm}
    \caption{
        Two-stage training using Policy Resonance and PPO-MA on FME with setting \textit{1A4B2C}.
        Policy Resonance (PR) is used in the second stage.
    }
    \label{fig:TwoStagePR-FME}
    \vspace{-0.3cm}
  \end{figure*}
\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ADCA-Two-Phase-Plus.pdf}
    \caption{
Training agents to cooperate in the ADCA environment using Conc4Hist implemented with PR. 
Policy Resonance (PR) is used in the second stage.
    }
    \vspace{-0.5cm}
    \label{fig:TwoStagePR-ADCA}
\end{figure*}


To key to addressing the DR problem is to find a better solution to deal with the multiagent version of the exploration-exploitation dilemma,
and eventually, we expect agents to diverge their behaviors and take explicit and well-divided responsibilities spontaneously.

The method we propose is Policy Resonance,
which is designed under the policy-based algorithm framework with the following features:
\begin{itemize}
    \item \textbf{The motivation is to modify the joint exploration behavior,
    so as to improve concurrent solutions against the exploration-exploitation dilemma.}
    \item Not task-specific, applicable to all MARL tasks.
    \item \textbf{Designed as a plugin module}. Not independent. Removable once training is done.
    \item Strictly \textbf{following the CTDE paradigm}. 
\end{itemize}

In current MARL models, 
an agent, without negotiating with other agents, has \textbf{full autonomy} to decide whether it should explore at any moment.
This practice is a convention directly inherited from the single-agent RL algorithm,
as in a single-agent RL task an agent has no one to cooperate with.
According to our DR problem analysis in Section \ref{sec:Analysis},
if we deliberately make agents reach tacit agreement on the opportunity to carry out exploitation or exploration,
the mutual exploration influence can be eliminated, therefore solving the DR problem.
Note that since exploration happens only in the centralized training (CT) stage,
we are not breaking the CTDE paradigm.

We use \textbf{policy resonance} to describe this tacit agreement on 
exploration-exploitation behaviors within a multiagent team.
As plugin implementation,
our approach is extended from the policy of the original RL model,
we use $\boldsymbol{\pi}=\lbrace \pi_1, \pi_2, \dots \rbrace$ to represent the raw joint policy,
where $\pi_i$ represents the raw individual policy of agent $i$.
After policy resonance is applied,
$\boldsymbol{\pi}$ will be mapped into a carefully designed joint policy $\boldsymbol{\pi}'$
which considers agent-wise synchronization on exploration-exploitation behaviors.
$\boldsymbol{\pi}' = \lbrace \pi_1', \pi_2', \dots \rbrace$.

When policy resonance is started, 
the new joint policy $\boldsymbol{\pi}$ will constantly and randomly switch between two states:
\textbf{resonated state} $\boldsymbol{\pi}'[\mathbf{u} | \varepsilon]$ and \textbf{non-resonated state} $\boldsymbol{\pi}'[\mathbf{u} | \overline{\varepsilon} ] $.
The selection of states is controlled by variable $\eta$ named \textbf{resonance probability},
the probability of choosing the resonated state is $P(\varepsilon)=1-P(\overline{\varepsilon})=\eta$, and:
\begin{equation}
    \label{eq:resonated}
        \boldsymbol{\pi}'[\mathbf{u}] = 
        P(\varepsilon)            \boldsymbol{\pi}'[\mathbf{u} | \varepsilon]  + 
        P(\overline{\varepsilon}) \boldsymbol{\pi}'[\mathbf{u} | \overline{\varepsilon} ] 
\end{equation}
The change of resonating state also influences each individual policy $\pi_i$:
\begin{equation}
    \label{eq:resonated-idv}
        {\pi}_i'({u_i}) = 
        P(\varepsilon)            {\pi}_i'({u_i} | \varepsilon)  + 
        P(\overline{\varepsilon}) {\pi}_i'({u_i} | \overline{\varepsilon} ) 
\end{equation}
\textbf{In non-resonated state}, agents make decisions autonomously and independently with individual policies $\lbrace \pi_1', \pi_2', \dots \rbrace$:
\begin{equation}\label{eq:non-resonated}
    \boldsymbol{\pi}'[\mathbf{u} | \overline{\varepsilon}]=\prod_{i=1}^{N} \pi_{i}^{\prime} ( u_{i} | \overline{\varepsilon})
\end{equation}
where $\pi_{i}^{\prime} ( u_{i} | \overline{\varepsilon})$ will be determined later.\\
\textbf{In resonated state}, agents will synchronously avoid exploration by exploiting current policies greedily:
\begin{equation}
    \label{resonatedindividual}
    \pi^{\prime}_i (u_i |   \varepsilon )=\left\{\begin{array}{ll}
        1, & u_i=u_i^* \\
        0, & \text{otherwise}
    \end{array}\right.
\end{equation}
\begin{equation}
\begin{split}
    \boldsymbol{\pi}'[\mathbf{u} |  \varepsilon]&=\left\{
        \begin{array}{ll}
            1, & \mathbf{u}=\mathbf{u}^{*} \\
            0, & \text{otherwise}
        \end{array}
        \right.
    % \\        
    % \mathbf{u}^{*} &= \lbrace u_1^*, u_2^*, \dots \rbrace \\
    % & = \lbrace \underset{u\in\mathcal{U}}{\mathrm{argmax}}[\pi_1(u )], \underset{u\in\mathcal{U}}{\mathrm{argmax}}[\pi_2(u)], \dots \rbrace
\end{split}
\end{equation}
where $\mathbf{u}^{*} = \lbrace u_1^*, u_2^*, \dots \rbrace$ is joint greedy action, 
and $u_i^* = {\operatorname{argmax}}_{u\in\mathcal{U}}[\pi_i(u)]$ is the most prefered action 
by current raw individual policy $\pi_i$.










Finally, 
we need to determine the mapping from raw individual policy $\pi_i$ to ${\pi}_i'({u_i} | \overline{\varepsilon})$.
Although policy resonance has done lots of modification on raw joint policy $\boldsymbol{\pi}$,
we can still \textbf{make individual policy invariant}, namely $\pi^{\prime}_i (u_i) = \pi_i (u_i)$.
In this way, 
this policy resonance process will be completely transparent to the host algorithms,
and will not damage the overall algorithm structure.
Combining  $\pi^{\prime}_i (u_i) = \pi_i (u_i)$ with Eq.\ref{eq:resonated-idv}:
\begin{equation}\label{eq:yyy1}
    \pi_i (u_i) = 
    \eta      {\pi}_i'({u_i} | \varepsilon)  + 
    (1-\eta)  {\pi}_i'({u_i} | \overline{\varepsilon} ) 
\end{equation}
Then from Eq.\ref{eq:yyy1} and Eq.\ref{resonatedindividual}:
\begin{equation}
    \label{eq:ff1}
    \pi^{\prime}_i (u_i |  \overline{\varepsilon}) = \left\{\begin{array}{ll}
        \frac{\pi_i(u_i^*)-\eta}{1-\eta}, & u_i=u_i^* \\
        \pi_i(u_i )\left[\frac{1-\pi^{\prime}_i \left(u_i^* |   \overline{\varepsilon}\right)}{1-\pi_i(u^*_i)}\right], & \text{otherwise}
    \end{array}\right.
\end{equation}
where $\frac{\pi_i(u_i^*)-\eta}{1-\eta}$ is abbreviated to $\pi^{\prime}_i \left(u_i^* |\overline{\varepsilon} \right)$ when $u_i \neq u_i^*$.

There is a constraint for $\eta$ from Eq.\ref{eq:ff1}.
Since $\pi^{\prime}_i(u_i |  \overline{\varepsilon}) \ge 0$, 
then $\eta$ needs to satisfy $\eta \le \pi_i(u_i^*)$.
E.g., when choosing between $n_k$ discrete actions, 
the minimum possible value of $ \underset{u_i}{\mathrm{max}} \pi_i(u_i)$ is $\frac{1}{n_k}$,
thus $\eta \in [0, \frac{1}{n_k}]$.

However, in practice we clamp $ \pi^{\prime}_i(u_i^* | \overline{\varepsilon}) $
to allow a larger resonance probability $\eta \in [0, 1)$, 
at the cost of precision in individual policy invariance constraint.
Enabling this clamping,
we improve Eq.\ref{eq:ff1} into:
\begin{equation}
    \label{eq:ff2}
    \pi^{\prime}_i (u_i |  \overline{\varepsilon}) = \left\{\begin{array}{ll}
        \max\left[p_{\min},  \frac{\pi_i(u_i^*)-\eta}{1-\eta} \right], & u_i=u_i^* \\
        \pi_i(u_i )\left[\frac{1-     \pi^{\prime}_i \left(u_i^* |\overline{\varepsilon} \right)   }{1-\pi_i(u^*_i)}\right], & \text{otherwise}
    \end{array}\right.
\end{equation}
where $p_{\min} \le \frac{1}{n_k}$ is a small constant to avoid the situation $\pi^{\prime}_i(u_i^*) < 0$,
and we abbreviate $\max\left[p_{\min},  \frac{\pi_i(u_i^*)-\eta}{1-\eta} \right]$ 
to $\pi^{\prime}_i \left(u_i^* |\overline{\varepsilon} \right)$ when $u_i \neq u_i^*$.


A pseudo of Policy Resonance is presented in Appendix \ref{sec:Pseudo}.
Depending on whether the resonance state is allowed to change within an episode,
there are two options available for the code-level implementation, as shown in Fig.~\ref{fig:PolicyResonance}, 
We use the episode-level resonance by default 
and a comparison of these two variants is provided in Appendix.
In our practice, a two-stage training procedure is used.
During the first stage Policy Resonance is not used ($\eta=0$),
then in the second stage $\eta$ gradually increased from 0 to $\eta_{max}$.
When the training is finished (or halted for testing),
all procedures related to Policy Resonance will be removed,
% restoring the decentralized decision-making (demanded by CTDE paradigm).
% then raw individual policies will take control back,
and then agents start to make decisions according to raw individual policies
in a decentralized way (required by the CTDE paradigm).




% \boldsymbol{\pi}'[\mathbf{u}] = 
% P(\varepsilon)            \boldsymbol{\pi}'[\mathbf{u} | \varepsilon]  + 
% P(\overline{\varepsilon}) \boldsymbol{\pi}'[\mathbf{u} | \overline{\varepsilon} ] 
% We hope this policy resonance procedure can be transparent to agent individuals,
% $\boldsymbol{\pi}'$ and $\pi_i'$ respectively,
% which introduces synchronised exploitation with a probability $\eta$.






% we design a new form of joint policy $\boldsymbol{\pi}' \neq \boldsymbol{\pi}$ to address the DR effect,
% while keeping the individual policies invariant 
% to avoid disturbing the host algorithms on which our method is implemented.
% This new joint policy $\boldsymbol{\pi}'$ randomly switches 
% between a normal state $\overline{\varepsilon}$ and a resonated state $\varepsilon$.
% The switching process is shown in Fig.~\ref{fig:PolicyResonance}, 
% the probability of choosing the resonated state is $P(\varepsilon)=1-P(\overline{\varepsilon})=\eta$.


% (1) Under the resonated state,
% the joint policy $\boldsymbol{\pi}'$ forces all agents to choose actions greedily.
% Each agent $i$ must select action 
% $u_i^* = {\operatorname{argmax}}_{u_i}[\pi_i(u_i )]$ that is prefered most by its current policy $\pi_i$.
% The joint greedy action of can be represented by $\mathbf{u}^*= \lbrace u^*_1,u^*_2,\dots ,u^*_N \rbrace$,
% and the resonated individual policy can be represented as:



% (2) Under the normal state, 
% each agent acts independently acoording to a non-resonated individual policy $\pi^{\prime}_i (u_i | \overline{\varepsilon})$.
% The non-resonated individual policy $\pi^{\prime}_i (u_i | \overline{\varepsilon})$ can be derived from $\pi_i (u_i)$
% using the invariance of individual policies:
% \begin{equation}
%     \label{eqinvariance}
%     \pi^{\prime}_i (u_i) = \pi_i (u_i)  \quad \Rightarrow \quad   P(\varepsilon) \pi^{\prime}_i(u_i |   \varepsilon) 
%     + P(\overline{\varepsilon}) \pi^{\prime}_i (u_i |  \overline{\varepsilon})  = \pi_i (u_i) 
% \end{equation}
% From Eq.~\ref{eqinvariance} and Eq.~\ref{resonatedindividual} we have:


% Due to the invariance of individual policies, 
% this resonance process is transparent to the host algorithms being implemented.
% Finally, from the global perspective of the team, 
% the new joint policy $\boldsymbol{\pi}'$ can be represented as: 



% agents explore the environment 
% we need to prevent agents from developing highly homogenous policies in scenarios such as the Lv-C level in FME.
% When necessary, we expect that agents can spontaneously
% diverge their behaviors to take explicit and well-divided responsibilities, 
% and eventually neutralize the DR effect.

% Nevertheless, blindly adding loss terms to drive agents to act differently is not an option.
% On the one hand,
% there are situations where all agents have to behave like one (FME Lv-A).
% On the other hand,
% it is hard to add limitations without reducing the MARL exploration efficiency and leading to a performance decay. 
% Moreover, a group of well-diverged behaviors does not necessarily mean 
% a group of agents acting differently at each decision step. 
% Firstly, some behavior is continuous and lasts for multiple decision steps.
% Secondly, two different behavior sequences may share a sub-sequence with identical actions. 




% The core inspiration is modifying the joint exploration behavior, 
% creating circumstances where agents cannot escape the consequences
% when they try to take chances and pass the responsibility to each other.
% To achieve this, we make an unprecedented modification to the way that
% individual policies compose into the joint team policy.

% In existing MARL works,
% the joint policy $\boldsymbol{\pi}$ is for each agent to make decisions independently:
% \begin{equation}
%     \boldsymbol{\pi}(\mathbf{u}|\mathbf{o}) =\prod_{i=1}^{N} \pi_i (u_i|o_{i})
% \end{equation}
% where the actions chosen by agents are refered to as $\mathbf{u} = \lbrace u_1,u_2,\dots  \rbrace$.
% The agent observations are represented by $\mathbf{o} = \lbrace o_1,o_2,\dots  \rbrace$, 
% which will be ommit for clearity from now on.

% Without breaking the framework of CTDE, in the centralized training stage,

% ***********************************
% Lib: spontaneous behavior divergence. 



==> 04ExperimentsAndResults.tex <==


\section{Experiments}

% the first-stage training can be viewed as a plain pre-training stage,
% preparing agent policies for the second-stage Policy Resonance.

% The second stage starts after learning from $M$ episodes.
% The Policy Resonance 
% begins with resonance probability $P(\varepsilon)=\eta=0$.
% Then $\eta$ increases linearly until it reaches the 
% a maximum probability $\eta_{max}$ in $M_{pr}$ episodes.
% Additionally, 
% for efficiency we only train parameters in the personality network
% and freeze other parameters in the policy network during the second stage.
% Ablations against this parameter-freezing can be found 
% in Fig.~\ref{fig:TwoStagePR} and \ref{fig:ADCAWithDifferentMethods}.



% In previous sections, 
% we analyzed the Diffusion of Responsibility (DR) effect in multiagent systems with 
% a simple multiagent task refered to as FME and explained the cause of the DR problem.
% Then a Policy Resonance (PR) method is proposed to solve the problem.
This section demonstrates the effectiveness of the Policy Resonance
approach on PPO-MA and Conc4Hist.
Experiments are performed using AMD x86 CPUs and Nvidia RTX8000 GPU.
% which are SOTA MARL algorithms.

\subsection{Setup.}
\begin{itemize}
    \item We use episode-level resonance as default 
    (comparison with the step-level variant is in Appendix \ref{appendix:compare-Resonance-level}).
    \item Agents use shared policy network parameters to promote training efficiency, 
    which is a useful technique commonly used by Qmix, Conc4Hist and PPO-MA, etc.
    \item Applying a two-stage training procedure. 
    During the first stage the Policy Resonance (PR) is not used, $\eta=0$.
    After $M$ episodes, the second stage begins with $\eta=0$, 
    linearly increasing $\eta$ to $\eta_{max}$ in $M_{pr}$ episodes.
    \item We designed another variant model called \textbf{PR-Fast}, 
    which adopts a parameter-freezing trick to accelerate training.
    Specifically, 
    we split agent policy nerual network into body network and head network.
    During the second stage in PR-Fast,
    body network parameters will be frozen to reduce computational cost.
    On the other hand, 
    the head network will be duplicated into $N$ copies for each agent, 
    allowing each individual to train their unique head network.
    \item The results demonstrated are obtained from repeated experiments launched by different random seeds 
    in all figures except Fig.\ref{fig:PersonalityDevelop},
    which is a special figure to illustrate six individual experiment cases.
    \item \textbf{PR is disabled when evaluating data such as win-rate and test reward}.
\end{itemize}

\subsubsection{FME Experiments.} As described in Section \ref{BenchmarkEnvironments}, 
tags like \textit{1A4B2C} are used to describe the setting of an FME task.
E.g., \textit{1A4B2C} is a task composed of
one Lv-A, four Lv-B, and two Lv-C levels.
The maximum reward expectation in each level is 1,
thus the maximum reward expectation of \textit{1A4B2C} is 7.
The number of the agents $N$ varies between $[3,40]$,
and there are $n_k=10$ available actions in each level.
For both PR and PR-Fast implementation,
the first pre-training stage lasts for $M=2^{18} \approx 260k$ episodes
because FME is very computational cheap.
Additionally, $\eta_{max}=0.75$ and $M_{pr}=50k$.
Other related hyper-parameters are listed in Appendix \ref{appendix:alg}.

\subsubsection{ADCA Experiments.}
In ADCA, an RL-controlled team with $N=50$ agents is trained  
to compete against an opposite team (controlled by script AI) with more agents $N' \in [120\%N, 160\%N]$.
We use Conc4Hist as the host algorithm.
Training in ADCA is computationally expensive,
requiring a day to train the first stage $M=83k$.
In the second stage, the PR hyper-parameters are selected as 
$\eta_{max}=0.75$ and $M_{pr}=6400$ to complete the second stage rapidly.
Other related details is shown in Appendix \ref{appendix:adca} and \ref{appendix:alg}.

\subsection{Main Result.}
\begin{figure}[!t]  
    \vspace{-0.6cm}
    \centering
    \includegraphics[width=0.65\linewidth]{img/DoRWithMoreAgentsNew.pdf}
    \vspace{-0.25cm}
    \caption{
        Evaluating PPO-MA, Fine-tuned Qmix, and PR-enhanced PPO-MA 
        in the FME diagnostic environment. FME setting is \textit{1A4B2C}.
        }
    \vspace{-0.5cm}
    \label{fig:DRWithMoreAgents}
\end{figure}

\begin{figure}[!t] 
    \centering
    \includegraphics[width=0.6\linewidth]{img/ADCA-MethodsNew.pdf}
    \vspace{-0.23cm}
    \caption{
        Win rates of algorithms tested in several ADCA settings.
        % The experiment is performed with several ADCA settings with different number of enemies. 
    %   The comparison of Conc4Hist without PR, 
    % training entire policy network with PR and training only personality head with PR.
    % The experiment is performed with several ADCA settings with different levels of hostile pressure.
    }
    \label{fig:ADCAWithDifferentMethods}
    \vspace{-0.5cm}
\end{figure}
\subsubsection{The Influence of Population Size $N$.}
The results of experiments on FME benchmark are displayed in Fig.\ref{fig:TwoStagePR-FME} and Fig.\ref{fig:DRWithMoreAgents}.
Note that the maximum reward expectation of \textit{1A4B2C} is 7, 
as is marked by dotted lines in these two figures.
It is apparent from Fig.\ref{fig:DRWithMoreAgents} that 
the DR problem causes a more significant impact as the number of agents grows larger.

Moreover, we can see that both Fine-tuned Qmix and PPO-MA suffer from the DR problem.
As a SOTA algorithm equipped with credit assignment (reward decomposition) techniques,
Fine-tuned Qmix can stand more agents than PPO-MA but still fails when $N \ge 15$.
\textbf{These results also indicate that credit assignment is not a solution to the DR problem}, 
because it does not change the exploration or exploitation behaviors of agents.

\subsubsection{The Effectiveness of Policy Resonance.}
Fig.\ref{fig:TwoStagePR-FME} and Fig.\ref{fig:TwoStagePR-ADCA} 
display the agents' learning process during the two-stage training process 
in FME benchmark and ADCA benchmark, respectively.
A reward breakthrough can be observed in both groups 
when PR is enabled at the beginning of the second stage.

Fig.\ref{fig:DRWithMoreAgents} and Fig.\ref{fig:ADCAWithDifferentMethods}
demonstrates the response of PR-enhanced algorithms towards 
the increase of agent population and task difficulty, respectively.
It can be seen in Fig.\ref{fig:DRWithMoreAgents} that PPO-MA implemented with PR
can easily outperform pure PPO-MA as well as Fine-tuned Qmix in FME.
Moreover, 
PPO-MA with PR can stably learn the optimal policy (dotted line in Fig.\ref{fig:DRWithMoreAgents})
even when $N \ge 30$.
For the ADCA benchmark,
Fig.\ref{fig:ADCAWithDifferentMethods} shows that 
Conc4Hist algorithm can promote the win rate from $50\%$ to above $80\%$ 
after implemented with PR under \textit{\footnotesize{120\%}-Enemy} setting.
In comparison, 
the performance of PR-Fast is slightly better.
PR-Fast can promotes \textit{\footnotesize{120\%}-Enemy} win-rate from $50\%$ to above $95\%$.
Even under very difficult \textit{\footnotesize{150\%}-Enemy} setting,
PR-Fast can still provide about 10\% win-rate improvement.

Furthermore, 
note that we do not need to identify DR problems before solving them.
We
\textbf{never assume or guess what form the DR problems might take in ADCA}.
Instead, 
we simply implement our PR approach on a proper host algorithm (Conc4Hist),
and then directly obtain a significant improvement.
This is because that PR is a general method and requires no task-specific knowledge.

% since PR is general and non-task-specific method a 
% Significant improvements can be observed in ADCA benchmark 
% from Fig.\ref{fig:TwoStagePR-ADCA} and Fig.\ref{fig:ADCAWithDifferentMethods}.
% the experiment with the number of enemies $N' \le 130\%N$.
% The win rate is promoted from less than $65\%$ to above $95\%$.
% When $N'\ge 140\%N$, 
% we can still observe solid improvement despite the surge in task difficulties.

% The results of algorithms implemented with and without Policy Resonance
% are shown in 
% can be compared with 
% Significant improvements can be observed in both groups when Policy Resonance 



% Results of this two-stage training process are presented in 
% Fig.~\ref{fig:TwoStagePR} and Fig.~\ref{fig:ADCAWithDifferentMethods}.
% A profound improvement is observed in 
% the experiment with the number of enemies $N' \le 130\%N$.
% The win rate is promoted from less than $65\%$ to above $95\%$.
% When $N'\ge 140\%N$, 
% we can still observe solid improvement despite the surge in task difficulties.
% Besides successfully demonstrating the effectiveness of our PR method,


\subsection{Ablations.}



\subsubsection{The Influence of $\eta$.}

\begin{figure}[!t]
    \vspace{-0.6cm}
    \begin{subfigure}{.49\linewidth}
      \centering
      % include first image
      \includegraphics[width=.8\linewidth]{img/abl_max_yita.pdf} 
      \caption{
        FME. \textit{1A4B2C}, $N$=30.
      }
      \label{fig:abla-eta-FME}
      \label{fig:DRWithMoreAgents2}
    \end{subfigure}
    \begin{subfigure}{.49\linewidth}
      \centering
      % include second image
      \includegraphics[width=.8\linewidth]{img/ADCA-Abl-EtaMax.pdf} 
      \caption{
        ADCA. $N$=50, $N'$=120\%$N$.
      }
      \label{fig:abla-eta-ADCA}
      \label{fig:BasicMALevels}
      
    \end{subfigure}
    \vspace{-0.25cm}
    \caption{The influence of $\eta_{max}$.}
      \label{fig:influence-eta}
      \vspace{-0.5cm}
\end{figure}
% \begin{figure}[!t]
%     \begin{minipage}{0.499\textwidth}
%         \centering
%         \vspace{-0.5cm}
%         \includegraphics[width=0.4\linewidth]{img/abl_max_yita.pdf}
%         \vspace{-0.25cm}
%         \caption{
%             The influence of $\eta_{max}$ in FME \textit{1A4B2C} task with $N=30$ agents.
%             }
%         \label{fig:abla-eta-FME}
%         \label{fig:DRWithMoreAgents2}
%     \end{minipage}\hfill
%     \begin{minipage}{0.499\textwidth}
%         \centering
%         \includegraphics[width=0.4\linewidth]{img/ADCA-Abl-EtaMax.pdf}
%         \vspace{-0.25cm}
%         \caption{
%             The influence of $\eta_{max}$ in ADCA task with $N=50$ agents against $N'=120\%N$ enemies.
%         }
%         \label{fig:abla-eta-ADCA}
%         \label{fig:BasicMALevels}
%     \end{minipage}
% \end{figure}



The resonance probability $\eta$ is manipulated by $\eta_{max}$.
We run ablation tests to study the influence of $\eta_{max}$.
The results in Fig.\ref{fig:influence-eta} 
suggests that $\eta_{max} \approx 0.75$ is a good option.


% \subsubsection{PR and PR-Fast.}
% In FME, PR and PR-Fast show no significant difference (Fig.\ref{fig:TwoStagePR-FME}),
% but in ADCA PR-Fast has advantage over PR (Fig.\ref{fig:ADCAWithDifferentMethods}).

\subsubsection{Step-Level PR and Episode-Level PR.}
The ablation study provided in Appendix \ref{appendix:compare-Resonance-level}
shows that they share almost identical performance.














% Besides Policy Resonance (PR),
% we also apply small modification on agents' policy network.
% The common practice is for all agents to share all network parameters,
% a cheap approach to significantly increase training efficiency.
% To decouple agent policies,
% we seperate the last few policy layers from the rest when PR stage begins,
% duplicating them so that each agent has its own unique policy head.
% However, alation experiments show little improvement is brought by this modification.

% -- GPU and CPU.

% \begin{figure}[!t]
%   \vspace{-0.75cm}
%   \centering
%   \includegraphics[width=0.77\linewidth]{img/BasicMAFindSignature.pdf}
%   \caption{
%       A signature that can be ultized to identify the DR effect.
%       Reward logged from training episodes becomes abnormally
%       higher than the real reward obtained during testing.
%       Replacing the value-base Qmix with the policy-based PPO-MA,
%       this signature still stands. 
%       }
%   \label{fig:BasicMAFindSignature}
%   \vspace{-0.5cm}
% \end{figure}

% \subsection{FME and ADCA Test Environment.}
% This paper uses the FME environment to investigate the effect of DR theoretically and experimentally.
% As introduced in previous sections,
% FME consists of three types of elemental levels.

% We use tags like \textit{1A4B2C} to describe the setting of a FME task, 
% e.g., \textit{1A4B2C} is a task composed of
% one Lv-A level, four Lv-B levels, and two Lv-C levels.
% With the maximum reward expectation in each level designed to be 1,
% we can effortlessly tell whether a policy reaches its optimal from the average test reward.

% FME is intentionally designed to limit the possible
% ways agents interact with each other to create convenience for analyzing agent behaviors and the DR effect.
% A question worth asking is whether the DR effect exists universally in other multiagent tasks,
% as real-world cooperative tasks are more sophisticated due to 
% the various ways that agents interact with each other.

% Therefore, we also use the ADCA (Asymmetric Decentralized Collective Assault,
% modified from \cite{fu2022concentration}) benchmark to 
% study the DR effect as well as test PR effectiveness.
% In ADCA, an RL-controlled team with $N=50$ agents is trained  
% to compete against an opposite team (controlled by script AI) with more agents $N' \in [120\%N, 160\%N]$.
% (Refer to supplemental materials for the details of ADCA.)
% In comparison, 
% FME has $N\in [3,40]$, 
% while the ADCA task has $N=50$ agents (100+ agents counting the enemies).
% FME is designed to limit the ways agents interact with each other for problem analysis,
% but ADCA depends on complicated agent-wise interaction to achieve team coordination.
% We can explain and imagine how the DR effect takes place in FME,
% however, 
% we have no clue about how the DR effect influences agents in ADCA.

% \subsection{Host MARL Algorithms.}
% Algorithms under testing are PPO-MA (similar to MAPPO \cite{yu2021surprising}), 
% Conc4Hist \cite{fu2022concentration} and fine-tuned Qmix \cite{hu2021rethinking}.
% There are significant differences between these algorithms,
% the former two algorithms are policy-based, on-policy models, 
% yet fine-tuned Qmix is a value-based, off-policy model with value-decomposition ability.
% The details of algorithms and training are provided in supplemental materials.



% \subsection{Influence of a Larger Agent Population.}
% According to our analysis in the previous section,
% the DR effect will cause a more significant impact on MARL performance when 
% the agent population grows larger.

% We test our hypothesis by running PPO-MA (policy-based) and 
% fine-tuned Qmix (value-based) on FME with the default setting \textit{1A4B2C}.
% % The number of the agents $N$ varies between $[3,40]$,
% % and there are $n_k=10$ available actions in each level.
% The FME setting \textit{1A4B2C} 
% has a maximum reward expectation $\mathbb{E}(R) = 7$ if
% agents can find the optimal policy for all $7$ levels.
% We anticipate that both algorithms should at least
% obtain $\mathbb{E}(R) \ge 5$ since 
% the ability to solve the Lv-A and four Lv-B levels 
% is fundamental for MARL algorithms,
% And the key concern is how algorithms 
% resolve two Lv-C levels.

% To exclude the influence of other factors that 
% may influence the performance of the MARL algorithms,
% we also test the performance of PPO-MA and fine-tuned Qmix
% on several other FME settings, including \textit{1A6B0C}, 
% \textit{1A5B1C} et.al.
% The number of agents remains at $N=30$ in this ablation experiment.


% Each experiment is repeated multiple times,
% using different random seeds,
% and 

% Since Lv-A and Lv-B levels are very foundamental,
% it is expected that MARL algorithms
% The ability to solve the Lv-A and Lv-B levels 
% is supposed to be foundamental for each MARL algorithms,
% As mentioned previously,
% the team  \textit{1A4B2C} the optimal reward is $7$.

% The results are demonstrated in Fig.~\ref{fig:DRWithMoreAgents} and Fig.~\ref{fig:BasicMALevels}.

% \subsection{The Growing DR Effect with The Increase of Agent Population}





% However, it is worth consideration this effect exists universally

% \subsection{The Signature of the DR Impact}

% To learn when measures should be taken to resolve the impact of the DR effect,
% we need to find the signature of DR's influence other than the performance decay.
% By carefully analyzing the data collected from the previous subsection,
% we find that if there are a higher proportion of Lv-C levels, 
% (which can trigger the DR effect according to the results above),
% the reward curves become abnormal.
% More specially, as can be observed from Fig.~\ref{fig:BasicMAFindSignature},
% as Lv-C levels gradually become the majority levels in FME settings,
% the distance between the test reward and the training reward becomes smaller,
% and eventually, their place is inverted.

% This phenomenon is algorithm-irrelevant, 
% since it can be observed in both value-based algorithm Qmix to policy-based algorithm PPO-MA,
% and it is highly correlated with the influence of the DR effect.
% As a result,
% this reward-inversion can be treated as a signature to identify the DR's impact.



% \subsection{The Effectiveness of Policy Resonance.}
% In general, we follow a two-stage approach to implement Policy Resonance (PR) on
% PPO-MA and Conc4Hist.

% Firstly, the policy neural networks of agents are modified,
% replacing the last layer with the personality network,
% as it is illustrated in Fig.~\ref{fig:PersonalityDivision}.
% Since the agent policies are trained from scratch,
% the training efficiency is also our concern.
% During the first stage, we freeze the personality network at the initial state,
% meaning that all agents still share all the policy parameters. 
% Also, Policy Resonance is not enabled at this stage.
% Therefore, 
% the first-stage training can be viewed as a plain pre-training stage,
% preparing agent policies for the second-stage Policy Resonance.

% The second stage starts after learning from $M$ episodes.
% The Policy Resonance 
% begins with resonance probability $P(\varepsilon)=\eta=0$.
% Then $\eta$ increases linearly until it reaches the 
% a maximum probability $\eta_{max}$ in $M_{pr}$ episodes.
% Additionally, 
% for efficiency we only train parameters in the personality network
% and freeze other parameters in the policy network during the second stage.
% Ablations against this parameter-freezing can be found 
% in Fig.~\ref{fig:TwoStagePR} and \ref{fig:ADCAWithDifferentMethods}.

% Our method is firstly applied on the FME \textit{1A4B2C} benchmark, 
% using PPO-MA as the host algorithm.
% Training in FME is very computational cheap, 
% usually taking less than 10 minutes to run $100k$ episodes.
% Therefore, we wait $M_{1st}=2^{18} \approx 260k$ episodes to ensure 
% that PPO-MA can improve the policies no more before beginning the second stage.
% Other PR hyper-parameters are $\eta_{max}=0.75$, and $M_{pr}=50k$.



% \subsection{Resolving the DR Problem in ADCA.}






% Training in ADCA is computationally expensive,
% taking about a day to train the first stage $M_{1st}=83k$
% and an hour to complete the second Policy Resonance stage. 
% Here we use Conc4Hist as the host algorithm to be enhanced,
% and test our PR method on 4 ADCA settings with different numbers of enemies $N' \in [120\%N, 160\%N]$.
% PR hyper-parameters are selected as $\eta_{max}=0.75$, and $M_{pr}=6400$ 
% to complete the second stage rapidly.


% Results of this two-stage training process are presented in 
% Fig.~\ref{fig:TwoStagePR} and Fig.~\ref{fig:ADCAWithDifferentMethods}.
% A profound improvement is observed in 
% the experiment with the number of enemies $N' \le 130\%N$.
% The win rate is promoted from less than $65\%$ to above $95\%$.
% When $N'\ge 140\%N$, 
% we can still observe solid improvement despite the surge in task difficulties.
% Besides successfully demonstrating the effectiveness of our PR method,
% a windfall we harvest in this experiment is the phenomenon that
% the win rate of Conc4Hist surprisingly rises in $N' \in [120\%N, 140\%N]$
% according to Fig.~\ref{fig:ADCAWithDifferentMethods}.
% This result once again reminds us 
% that the impact of the DR effect is difficult to predict,
% and not precisely relevant to the task difficulty which is defined by us as humans.



% The advantage of FME is its simplicity, 
% which creates convenience for the analysis of agent behaviors and 
% RL algorithm tendencies.
% However, 
% FME is intentionally designed to limit the possible
% ways that agents can influence each other.
% A question worth asking is that 
% whether the effect DR exists universally in other multiagent tasks.
% Because compared with FME,
% some cooperative tasks are exponentially more sophisticated due to 
% the diversed way that agents interact with each other.

% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 



% On the one hand,
% the personality network begins to divide in a way
% shown in Fig.~\ref{PersonalityDivision} and
% is progammed to complete all the divisions in $M_{pd}$ network updates,
% assigning all agents with an unique personality network.
% we do not adopt Policy Resonance approach and 
% freeze the personality network to its root.
% In other words, all agents share the same personality network.
% The first stage is identical to the original training procedure of PPO-MA and Conc4Hist.





% During the first step, 
% the training is 


% The first stage is responsible to train agents 

% The first stage is almost identical to the original training of PPO-MA and Conc4Hist,
% except that a personality network is inserted at the head of the agent policy network.

% In the first stage,
% the policy head (last few layers of the policy neural network) of agents is replaced the personality network.
% Since our models are trained from the scratch, 
% sample efficiency is essential for 
% During the entire stage, agents share the root personality nerwork
% to reduce the policy parameter space.





% a personality network is implemented at the head of the agent policy network,
% replacing 
% Everything works identical with the original training process,
% except that the agent policy network
% a personality network is inserted at the head of the agent policy network.
% but a inserted personality network
% except a personality network
% the head of the policy 


% \begin{figure}[!t] 
%   \vspace{-0.5cm}
%   \begin{minipage}{0.5\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{img/BasicMALevels-crop.pdf}
%       \caption{The comparison of policy-based algorithms and value-based algorithms under several FME settings.
%       Both algorithms significantly suffer from the DR effect caused by Lv-C levels.
%       % All basicMA tasks share the same optimal reward expectation $R=7$, marked as blue dotted lines.
%       % It is clear that both models significantly suffer from the DR effect caused mainly by Lv-C levels,
%       % and fail to reach the optimal reward when Lv-C levels are present.
%       }
%       \label{fig:BasicMALevels}



%   \end{minipage}
% \end{figure}






% \begin{figure}[!t]
%   \vspace{-0.7cm}
%       \centering
%       \includegraphics[width=0.5\linewidth]{img/ADCA.jpg}
%       \caption{The Asymmetric Decentralized Collective Assault (ADCA) benchmark.
%       % MARL algorithm needs to win the enemy team with quantitative and information advantages.
%       }
%       \label{fig:ADCA}
% \end{figure}




==> 11apendix_real.tex <==



\appendix
\newpage
\section{Appendix}
\subsection{Lv-B Optimal Reward Expectation.} \label{lvb-reward}

In Lv-B the team is rewarded according to number of agents selecting arm $u^\beta$, 
namely $R_B=N_{\mathcal{A}}(u^\beta)/N*c_\beta$.
Here $N_{\mathcal{A}}(u^\beta)$ counts the number of agents selecting $u^\beta$, 
$c_\beta$ is a constant making the optimal reward expectation fixed to 1. 
Let $u^{\beta*}= \underset{u}{\mathrm{argmax}}  [p_\beta(u)]$,
then $c_\beta=1/{\underset{u}{\mathrm{max}}[p_\beta(u)]}=1/ {p_\beta(u^{\beta*})}$.
Let $\boldsymbol{\pi} = \lbrace \pi_1,\pi_2, \dots \rbrace$ be the joint policy,
then the reward expectation is:
\begin{equation}
    \label{eq:typeb-expect}
    \begin{aligned}
    \mathbb{E}\left[R_B|\boldsymbol{\pi}\right] 
    &=\Sigma_{i} \Sigma_{k} {\pi_{i}\left(u^{k}\right) 
    p_{\beta}\left(u^{k}\right)} c_{\beta}/{N} \\
    &=c_{\beta} \Sigma_{k} p_{\beta}\left(u^{k}\right)  {\Sigma_{i} 
    \pi_{i}\left(u^{k}\right)}/{N}  \\
    &\leq c_{\beta} p_{\beta}\left(u^{\beta*}\right) 
     {\Sigma_{k} \Sigma_{i} \pi_{i}\left(u^{k}\right)}/{N} 
    % \leq c_{\beta} p_{\beta}\left(u^{\beta*}\right)=1
    \leq 1
    \end{aligned}
    \end{equation}
where $\pi_{i}\left(u^{k}\right)$ represents the probability of $i$-th agent choosing action $u^k \in \mathcal{U}$.
The optimal solution is all agents chosing $u^{\beta*}$, which is the condition for equality in Eq.\ref{eq:typeb-expect}.


\subsection{Details of FME.}\label{appendix:FMEtable}
In this paper, 
the FME environment is used to investigate the DR problem.
Each FME task is composed of a series of levels,
and at each level, agents need to make single-step decisions before entering the next one.
The team reward obtained at a level is immediately given to RL algorithms for policy optimization.

As described previously, there are three types of levels in FME.
One type of level can be used multiple time in a task,
as we can make them different by changing the configuration.
E.g., in the first Lv-B level of our \textit{1A2B4C} task,
the actions with top probability to be rewarded is: 
\begin{itemize}
    \item Lv-B configuration \textit{Act-5-6-7}:  50\% \textit{Act-5} ;  40\% \textit{Act-6}  ;  10\% \textit{Act-7}
\end{itemize}
but the second Lv-B level has an alternative configuration: 
\begin{itemize}
    \item Lv-B configuration \textit{Act-6-7-8}:  50\% \textit{Act-6} ;  40\% \textit{Act-7}  ;  10\% \textit{Act-8}
\end{itemize}
Moreover, the main action in Lv-A levels and Lv-C levels
can be configured differently. 
E.g., if Act-0 is set as the main action $u^\alpha$ in an Lv-A level,
then Act-1, Act-2 et.al. will be regarded as non-main actions in $u^{\alpha}$.

All duplicated levels are given different configurations
to avoid potential mutual influence during training.
Configurations of all FME settings used in experiments are listed in Tabel.~\ref{basicma_configurations}.

\begin{table*}
	\caption{
        The level configurations of each tagged FME task are used in this paper ($n_k \ge 10$).
        For Lv-A and Lv-C levels, this table gives the selection of the main action $u^\alpha$ or $u^\gamma$, e.g. \textit{Act-0}.
        For Lv-B levels, a action sequence is provided, 
        e.g., \textit{Act-4-5-6} indicate that the probability of rewarding \textit{Act-4}, \textit{Act-5}, \textit{Act-6} is 50\%, 40\%, 10\% respectively.
        The probability descent pattern is fixed to $[50\%, 40\%, 10\%]$ in all Lv-B configurations.
        The reward expectation of an optimal learned policy $\mathbb{E}\left[R|\boldsymbol{\pi}^*\right]$ 
        equals to the number of levels in these tasks.
	}
	\label{basicma_configurations}
	\centering
	\setlength{\tabcolsep}{1.5mm}{
		\begin{tabular}{cccccccc}
		\toprule
	 & \textbf{1A6B0C}                           
	 & \textbf{1A5B1C}                           
	 & \textbf{1A4B2C}                           
	 & \textbf{1A3B3C}                           
	 & \textbf{1A2B4C}                           
	 & \textbf{1A1B5C}                           
	 & \textbf{1A0B6C}  \\
		\midrule
		Lv.1   & Act-0                             & Act-0                             & Act-0                             & Act-0                             & Act-0                             & Act-0                             & Act-0    \\
		Lv.2   & Act-4-5-6 & Act-4-5-6 & Act-5-6-7 & Act-5-6-7 & Act-5-6-7 & Act-5-6-7 & Act-0    \\
		Lv.3   & Act-5-6-7 & Act-5-6-7 & Act-6-7-8 & Act-6-7-8 & Act-6-7-8 & Act-0                             & Act-1    \\
		Lv.4   & Act-6-7-8 & Act-6-7-8 & Act-7-8-9 & Act-7-8-9 & Act-0                             & Act-1                             & Act-2    \\
		Lv.5   & Act-7-8-9 & Act-7-8-9 & Act-8-9-5 & Act-0                             & Act-1                             & Act-2                             & Act-3    \\
		Lv.6   & Act-8-9-0 & Act-8-9-5 & Act-1                             & Act-1                             & Act-2                             & Act-3                             & Act-4    \\
		Lv.7   & Act-9-0-1 & Act-0                             & Act-0                             & Act-2                             & Act-3                             & Act-4                             & Act-5   \\
		\midrule
		$\mathbb{E}\left[R|\boldsymbol{\pi}^*\right]$  & 7.0 & 7.0  & 7.0 & 7.0 & 7.0    & 7.0      & 7.0   \\
		\bottomrule
	\end{tabular}}
	
	\end{table*}




	% 今天晚上 新增了eta max消融重复实验
	% 新增了原始conc4hist实验
	% 新增了二阶段conc4hist实验

\subsection{Details of ADCA.}\label{appendix:adca}

In the straightforward FME environment,
we can at least identify and understand 
the exact problem (the Lv-C levels) and behaviors that cause the DR effect.
Nevertheless,
most multiagent tasks cannot be decomposed and analyzed that easily.
When the multiagent system becomes large and chaotic,
identifying all behavior combinations involving agent-wise cooperation becomes almost impossible.
Thus, distinguishing behaviors that 
are vulnerable to the DR effect is hardly possible in such systems.
In other words,
the DR effect may appear in complex forms beyond our comprehension.


The Asymmetric Decentralized Collective Assault (ADCA)
benchmark is a swarm combat environment modified and 
improved from \cite{fu2022concentration}.
As shown in Fig.\ref{fig:TwoStagePR-ADCA}, in ADCA, 
two asymmetric teams compete with each other,
the RL-controlled team has $N=50$ agents and suffers from
limited observation as well as observation interference.
On the other hand, 
the opposite team that is controlled by script AI
has much more agents to use ($N' \in [120\%N, 160\%N]$),
observes all the field information for making decisions
and has faster weapon targeting speed.

All agents control their movement by adjusting the direction 
of their acceleration.
Discrete actions available to agents are responsible
for selecting acceleration and rotating weapon directions.
To address the challenge of outnumbered situation and jammed observation,
the team needs to learn to strike back by taking terrain advantages,
which slightly increases the effective weapon range.
Agents are rewarded according to their kill-death ratio.
The winning condition is to eliminate all opponents,
or at least to reverse the disadvantage in agent number 
when time is up.


\subsection{DR Problem: Policy-Based Perspective.} \label{Policy-Based-Perspective}
In this section, we interpret DR from an individual perspective,
and explain that staying in a team with a larger agent population $N$
can lead to a requirement for exponentially more samples,
which is necessary before an agent can learn proper behaviors against the DR effect.


Here we still use an Lv-C level in FME for analysis.
Let $b_{-i}(u^\gamma | \boldsymbol{\pi}) = \sum_{j=1,j\neq i}^N \pi_j(u^\gamma)$ be the policy baseline \cite{williams1992simple},
the advantage \cite{schulman2015high} of choosing $u^\gamma$ for an agent $i$ can be represented by:
\begin{equation}
	\label{eq:pbDR2}
	% \text{Advantage}(u^\gamma)= - \left[ \sum_{j=1,j  i}^N \pi_j(u^\gamma) \right]
\text{Advantage}(u^\gamma) = -p_{-i}(u^\gamma|\boldsymbol{\pi})  b_{-i}(u^\gamma|\boldsymbol{\pi}) + \frac {1-p_{-i}(u^\gamma|\boldsymbol{\pi})} {N-1}
	\end{equation}
where $p_{-i}(u^\gamma|\boldsymbol{\pi}) = \prod_{j=1,j\neq i}^N \pi_j(u^\gamma)$ is the probability of all agents
except $i$ selecting the main action $u^\gamma$.
To correctly estimate Eq.~\ref{eq:pbDR2}, 
agents have to collect at least one episode that is punished due to abandoning $u_{-\gamma}$.
Let $M_{tot}$ be the number of episode we have collected,
$M\approx  \pi_i(u^\gamma)M_{tot}$ be the number of episodes 
in which agent $i$ selected $u^\gamma$,
and $M_{pen}$ be the number of episodes in which the team receives penalty.
Then we have:
\begin{equation}
	\mathbb{E}(M_{pen}|\boldsymbol{\pi}) = M p_{-i}(u^\gamma) =  M \prod_{j=1,j\neq i}^N \pi_j(u^\gamma)
\end{equation}
To expect at least one negative example for selecting the main action $\mathbb{E}(M_{pen}) \ge 1$,
we need to collect 
$M \ge \prod_{j=1,j\neq i}^N \pi_j(u^\gamma)^{-1}$ episodes before training,
which grows exponentially larger when $N$ increases.
This awkwardness can be resolved when most agents are already 
stabilized at a deterministic policy with $\pi_j \approx 1$,
but it is not allowed by regularization terms designed to maintain the agent exploration. 
As a result,
it is impossible for agents to estimate Eq.~\ref{eq:pbDR2} correctly when $N$ is large,
causing agents to overestimate $\text{Advantage}(u^\gamma)$ and continually developing preference in $u_{\gamma}$.


\begin{figure*}[!t]
	\centering
	\includegraphics[width=\linewidth]{img/EpisodeLevelStepLevelCompare.pdf}
	\caption{
        Comparing episode-level and step-level Policy Resonance in FME.
        The setting is \textit{1A4B2C}, $N=30$ and $n_k=10$.
	}
	\label{fig:EpisodeLevelStepLevelCompare}
\end{figure*}

\subsection{DR in Value-Based Methods.}
The analysis of the DR effect in value-based Methods is easier.
The exploration of most value-based RL methods is powered by $\epsilon$-greedy 
for carrying out exploration.
To guarantee that agents can always discover other possible policies better than the current ones,
agents always have a small probability of acting against the advice of value functions (Q functions).
Suppose there are $n_k$ discrete actions in FME Lv-C level, 
and all agents mistakenly value the main action $u^\gamma$ more than other actions,
then the probability for agents to notice this mistake in an episode is:
\begin{equation}
    P_{penalty} = \left[(1 - \epsilon) + \frac{\epsilon}{n_k} \right]^N 
\end{equation}
where $(1 - \epsilon) + \frac{\epsilon}{n_k} < 1$,
and $P_{penalty}$ will decrease exponentially with the $N$ becomes larger.
When the agent population is large enough,
the agents will mistakely treat ALL-$u^\gamma$ policy as a sub-optimal solution
to finish the task,
with each individual expecting some other agents to take the responsibility
to carry out non-main actions.
This theory is backed by experiment results shown in Fig.~\ref{fig:BasicMALevels},
where the fine-tuned Qmix \cite{rashid2018qmix, hu2021rethinking}, a well-developed value decomposition method,
is used to solve the FME tasks.
Qmix fails when $N$ is large and numerous Lv-C levels are present.




\input{12apendix_code.tex}



\subsection{MARL Algorithms Used in Experiments.}\label{appendix:alg}

PPO-MA is an algorithm that resembles much of the MAPPO model proposed in \cite{yu2021surprising}.
However, 
most tricks used in \cite{yu2021surprising} are not adopted to keep the model as simple as possible, e.g., the trick of action masking and input shaping.
Moreover, we used dual-clip PPO \cite{ye2020mastering} instead of the classic version
to increase training stability.

Conc4Hist is a model based on the Concentration Network proposed in \cite{fu2022concentration}.
This model is efficient in dealing with large-scale multiagent problems and
can consider multi-step observation to work against interference 
that may exist in sophisticated MARL environments.

Fine-tuned Qmix is a value decomposition algorithm specialized in solving 
small-scale cooperative multiagent tasks such as SMAC.
In \cite{hu2021rethinking} the authors discovered that 
code-level implementation tricks significantly influence the performance of Qmix.
After tuning, Qmix surprisingly outperforms 
many SOTA methods in the value-decomposition MARL algorithm family.

There are significant differences between these algorithms,
First and most importantly,
the former two algorithms are policy-based, but Qmix is value-based.
Secondly, 
Qmix should be categorized into off-policy models while 
the former two algorithms are on-policy models considering 
how they utilize the collected samples.
Thirdly,
Qmix is designed with the function of breaking down team rewards
into individual rewards,
while PPO-MA and Conc4Hist simply dispense team rewards equally to each agent.
When individual rewards are not available, e.g., in FME.
The details of the hyper-parameters for each algorithm are shown in Table.~\ref{hyper-para}.
\input{h-table.tex}



\subsection{Ablations of the Resonance Probability.}
As the core hyper-parameter in Policy Resonance,
the resonance probability $\eta$ is our primary concern during Policy Resonance.
We carry out an ablation study of $\eta$ by changing the maximum $\eta$ limit $\eta_{max}$.
Recall that $\eta$ increase from 0 to $\eta_{max}$ in $M_{pr}$ episodes,
then maintains at $\eta_{max}$ till the end of training.
We set the $M_{pr}$ value identical to previous experiments,
and the impact of shifting $\eta_{max}$ is illustrated in 
Fig.~\ref{fig:DRWithMoreAgents2} and Fig.~\ref{fig:BasicMALevels}.

In both FME and ADCA,
a great leap in performance is observed even when the $\eta_{max}$ is as low as $0.1$.
Nevertheless, a larger $\eta_{max}$ setting around $0.7$ 
reduces the test reward variance (when experimented repeatedly) in FME,
and benefits the winning rate in ADCA.




\subsection{Ablations of PR and PR-Fast.}
In the Policy Resonance stage, it is not necessary to train the whole policy neural network,
instead, 
freezing the shared parameters that are not processed by the policy head networks
can accelerate the learning process.
To verify the influence of the two method variants,
we provide a comparison study in both PPO-MA and ADCA tasks.


Fig.~\ref{fig:TwoStagePR-FME} and \ref{fig:ADCAWithDifferentMethods} demonstrate the comparison of 
the performance differences depending on whether or not to freeze the shared parameters.
In PPO-MA tasks,
the difference between the two method variants is insignificant.
In contrast,
this parameter freezing technique plays a vital role in promoting the winning rate in ADCA.



% \subsection{Relationship between DR Effect and its Signature.}
% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=\linewidth]{img/SignitureADCA.pdf}
% 	\caption{
% 		In multiple ADCA tasks, the similar but abnormal reward reversion is also observed,
% 		which can be treated as a signature of the DR effect.
% 		This figure only captures the early phase of training (0 to 20k episodes) 
% 		in order to illustrate the way that reward curves become inverted during training.
% 	}
% 	\label{fig:SignitureADCA}
% \end{figure}


% Fig.\ref{fig:BasicMAFindSignature} reveals 
% that the reward-inversion signature only emerges 
% when the DR effect is causing considerable negative impact.
% Combining the results from 
% Fig.\ref{fig:BasicMAFindSignature} and \ref{fig:SignitureADCA},
% it is clear that this signature stands still 
% when we switch between three different algorithms and
% two distinct test environments.

% In the previous discussion,
% we trace the source of the DR effect back to the exploration-exploitation dilemma.
% Taking this dilemma into consideration,
% our hypothesis on the relationship between the DR effect and its signature is as follows.

% RL algorithms, no matter policy-based or value-based, need to adopt exploration measures
% for policy discovery and optimization.
% But these measures are initially designed in single-RL algorithms
% without considering agent-wise influences.
% These exploration measures accidentally shield agents in a large team against
% the penalty caused by the lack of diverged personality required by tasks.
% Unfortunately, after the training is done and exploration measures are removed,
% the weakness of lacking a clear responsibility division 
% is eventually exposed by the testing episodes.

% Here it is worth mentioning that even if the exploration measures are not removed in testing,
% the agent policies are still far from being able to meet the task requirements.
% Firstly, the policies are already poisoned by the DR effect during training.
% Secondly, if the exploration measures are not removed, 
% even the classic tasks like Lv-A have to suffer from the collateral damage of this scheme.





==> old_intro.tex <==
Next, we put forward our solution to solve multiagent DR problem by pushing agents
to develop personality, we name this process as Policy Resonance.
Policy Resonance solve the problem from two aspect,
both takes place during the stage of centralized training in the paradigm
of CTDE (Centralized Training with Decentralized Execution).

First, providing the infrastructure to achieve complicated personality.
each agent need to has a part of private neural network.
But unluckily, this will dramatically reduce RL efficiency.
To deal with this, we propose training agents 
following a tree of personality. 
At the begining, all agents share the same root personality as their private network.
As the training goes on, 
agents gradually and randomly split up their personalities, 
just like a tree developing more and more branches from its root.
Untill eventually, 
each agent has an unique private personality sharing with no one else.
But as we mentioned earlier, 
there is a long way between having the infrastructure to develop personalities 
and actually developing them.
The model will not work untill we push agents to find the personalities of their own.

Second, driving agents to find the personalities of their own.
In preliminary experiments, we tried many ways that is easy to come by,
including forcing agent-wise policy KL-divergence,
skip connecting agents' one-hot identity everywhere in policy neural network to remind it of its uniqueness, 
shaping intrinsic rewards,
removing (or reversing the sign of) the entropy loss term in policy-based algorithm et.al..
Those methods indeed make agents act differently, 
however, also make agents act blindly with no consideration about the task itself, 
resulting in fake personalities with no help in solving the task.
Eventually, we have to use a bold and unprecedented method that we called Coercive Policy Resonance.
More specially, 
we manipulate joint policy but keep the individual agent policy $\pi$ untouched during training,
bending the joint policy to help develop 
distinct individual personalities only when necessary and helpful to promote cooperation.

In experiment section, 
We demonstrates that the DR effect is general in MARL.
From simple few-step games to sophisticated large-scale combat environments,
from policy-based methods to value-based methods,
the influence of the DR effect is very common and can be effectively tackle with 
by proposed Policy Resonance methods.


==> old_resounance.tex <==
(2) Under the normal state,
each agent acts indenpendently acoording to a revised individual policy $\pi^{\prime}_i (u_i | \overline{\varepsilon})$.
Furthermore, we need to ensure that the combined individual policy $\pi^{\prime}_i(u_i)$ stay invariant,
% This revised individual policy needs to stay identical to the original individual policy $\pi_i(u_i)$,
% in such we our PR implemention becomes tranparent to the original algorithms
in such way we can avoid influencing host algorithms after implemented by our method,
making Policy Resonance a transparent procedure from the view of the host algorithms:
% has to be designed to satisfy the invariance of individual policy:
\begin{equation}
	\label{eqinvariance}
	\pi^{\prime}_i (u_i) = P(\varepsilon) \pi^{\prime}_i(u_i |   \varepsilon) 
	+ P(\overline{\varepsilon}) \pi^{\prime}_i (u_i |  \overline{\varepsilon}) 
	= \pi_i (u_i)
\end{equation}
From Eq.~\ref{eqinvariance} and Eq.~\ref{resonatedindividual}, the revised individual policy without resonance can be obtained:
\begin{equation}
	\label{eq:raw}
	\pi^{\prime}_i (u_i |  \overline{\varepsilon}) = \left\{\begin{array}{ll}
		\frac{\pi_i(u_i^*)-\eta}{1-\eta}, & u_i=u_i^* \\
		\pi_i(u_i )\left[\frac{1-\pi^{\prime}_i \left[u_i^* |   \overline{\varepsilon}\right]}{1-\pi_i(u^*_i)}\right], & \text{otherwise}
	\end{array}\right.
\end{equation}
However, there is a hidden constraint for resonance probability $\eta$ from Eq.\ref{eq:raw}.
Since $\pi^{\prime}_i(u_i |  \overline{\varepsilon}) \ge 0$ for $\forall u_i$, then $\eta \le \pi_i(u_i^*)$.
For example, in the case of chosing between $n_u$ discrete actions, 
it is required that $\eta \le \operatorname{min} \pi_i(u_i^*) = 1/n_u \le \pi_i(u_i^*)$.
Nevertheless, 
in practice we can clamp the value of $ \pi^{\prime}_i(u_i^* | \overline{\varepsilon}) $
to allow a larger resonance probability $\eta$, 
at very little cost of precision in individual policy invariance,
if so, the first part of Eq.\ref{eq:raw} becomes:
\begin{equation}
	\pi^{\prime}_i (u_i=u_i^* |  \overline{\varepsilon} ) = 
		max\left(p_{opm},  \frac{\pi_i(u_i^*)-\eta}{1-\eta} \right)
\end{equation}
where $0 < p_{opm} \le \operatorname{min} \pi_i(u_i^*) = 1/n_u$ is a small constant to avoid
the situation in which $\pi^{\prime}_i(u_i^*) < 0$.

Finally, from the team's perspective, the new joint policy $\boldsymbol{\pi}'$ can be represented as: 
\begin{equation}
	\label{eq:resonated}
		\boldsymbol{\pi}'[\mathbf{u}] = 
		P(\varepsilon)            \boldsymbol{\pi}'[\mathbf{u} | \varepsilon]  + 
		P(\overline{\varepsilon}) \boldsymbol{\pi}'[\mathbf{u} | \overline{\varepsilon} ] 
	\end{equation}
	\begin{equation}
		\boldsymbol{\pi}'[\mathbf{u} |  \varepsilon]=\left\{\begin{array}{ll}
		1, & \mathbf{u}=\mathbf{u}^{*} \\
		0, & \text { otherwise }
		\end{array}, 
		\quad \boldsymbol{\pi}'[\mathbf{u} | \overline{\varepsilon}]=\prod_{i=1}^{N} 
		\pi_{i}^{\prime} ( u_{i} | \overline{\varepsilon})\right.
		\end{equation}
Also, there are two ways provided in Fig.~\ref{fig:PolicyResonance}, 
determining on whether the resonance state should be changed within a episode.
We use the episode-level resonance by default and ablation studies is provided in supplemental materials. 



==> temp.tex <==
\begin{figure*}[!t]
    \vspace{-1cm}

    \begin{minipage}{0.3\textwidth}
    \centering
        \includegraphics[width=\linewidth]{img/DoRWithMoreAgentsNew.pdf}
        \caption{Evaluating PPO-MA, Fine-tuned Qmix, and PR-enhanced PPO-MA 
        in the FME diagnostic environment. FME setting is \textit{1A4B2C}.}
        \label{fig:DRWithMoreAgents}
    \end{minipage}\hfill
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{img/ADCA-MethodsNew.pdf}
        \caption{Win rates of algorithms tested in several ADCA settings.}
        \label{fig:ADCAWithDifferentMethods}
    \end{minipage}\hfill
    \begin{minipage}{0.2\textwidth}
        \centering
        \includegraphics[width=\linewidth]{img/abl_max_yita.pdf}
        \caption{The influence of $\eta_{max}$ in FME \textit{1A4B2C} task with $N=30$ agents.}
        \label{fig:abla-eta-FME}
        \label{fig:DRWithMoreAgents2}
    \end{minipage}\hfill
    \begin{minipage}{0.2\textwidth}
        \centering
        \includegraphics[width=\linewidth]{img/ADCA-Abl-EtaMax.pdf}
        \caption{
            The influence of $\eta_{max}$ in ADCA task with $N=50$ agents against $N'=120\%N$ enemies.
        }
        \label{fig:abla-eta-ADCA}
        \label{fig:BasicMALevels}
    \end{minipage}
    \vspace{-0.5cm}
\end{figure*}


% <!-- and reveal its similarity to a social psychology phenomenon known as the bystander % effect.
% Second, -->
